Pseudo-RIS: Distinctive Pseudo-supervision Generation for Referring Image Segmentation

We propose a new framework that automatically generates high-quality segmentation masks with their referring expressions as pseudo supervisions for referring image segmentation (RIS). These pseudo supervisions allow the training of any supervised RIS methods without the cost of manual labeling. To achieve this, we incorporate existing segmentation and image captioning foundation models, leveraging their broad generalization capabilities. However, the naive incorporation of these models may generate non-distinctive expressions that do not distinctively refer to the target masks. To address this challenge, we propose two-fold strategies that generate distinctive captions: 1) 'distinctive caption sampling', a new decoding method for the captioning model, to generate multiple expression candidates with detailed words focusing on the target. 2) 'distinctiveness-based text filtering' to further validate the candidates and filter out those with a low level of distinctiveness. These two strategies ensure that the generated text supervisions can distinguish the target from other objects, making them appropriate for the RIS annotations. Our method significantly outperforms both weakly and zero-shot SoTA methods on the RIS benchmark datasets. It also surpasses fully supervised methods in unseen domains, proving its capability to tackle the open-world challenge within RIS. Furthermore, integrating our method with human annotations yields further improvements, highlighting its potential in semi-supervised learning applications.

==> reb_tables/analysis_caption.tex <==
\vspace{-0.6cm}
\begin{table}[h]
    \centering
    \scriptsize
    \caption{\footnotesize{Statistics of our captions compared to GT expressions.}}
    \begin{tabular}{@{\hspace{7pt}}l@{\hspace{6pt}}|c@{\hspace{6pt}}c@{\hspace{6pt}}c@{\hspace{6pt}}c@{\hspace{6pt}}}
    \hline
        Statistics & Ours &RefCOCO & RefCOCO+ & RefCOCOg \\ \hline
       \# of Vocabulary & 37,588 & 9,342 & 11,090 & 11,710 \\
       \# of Average Length & 9.44 & 3.61 & 3.53 & 8.43 \\
       \# of Average Objects & 3.14 & 2.50 & 2.49 & 1.93 \\
       \# of Average Expressions & 14.48 & 2.84  & 2.84 & 1.91 \\
       % \# of Average CLIPscore & & & & \\
       % \# of Average Noun & & & & \\
    \hline
    \end{tabular}
    \label{reb_tab:analysis_caption}
\end{table}
\vspace{-0.2cm}

==> reb_tables/captioning_models.tex <==
\vspace{-0.5cm}
\begin{table}[h]
    \centering
    \scriptsize
    \caption{\footnotesize{mIoU results with other caption models in ours on RefCOCOg. *) Mokadi et al., ClipCap: CLIP Prefix for Image Captioning, arXiv 2021.}}
    \begin{tabular}{lll|ccc}
    \hline
    Models & Params & Trained data & val(U) & test(U) & test(G) \\ \hline
    ClipCap* & 0.15B & CC3M & 41.50 & 42.21 & 42.32 \\
    CoCa  & 2.1B & LAION-5B + CC3M & 45.99 & 46.67 & 46.80 \\
    CoCa & 2.1B & LAION-5B + COCO & 47.23 & 47.90  & 47.94 \\ \hline
    % CLIPCAP & COCO & - & - & - \\ \hline
    \end{tabular}
    \label{reb_tab:captioning_models}
\end{table}
\vspace{-0.3cm}

==> reb_tables/cross_domain.tex <==
% \begin{table}[]
%     \centering
%     \small
%     \caption{\textcolor{red}{R2: Cross-domain}}
%     \begin{tabular}{c|cccc}
%     \hline
%     Domains     &  PhraseCut & RefCOCO & RefCOCO+ & RefCOCOg\\ \hline
%     Visual     & 1203 classes & 80 classes & 80 classes & 80 classes \\
%     Textual & template & Positional + Short & Short & Long + Complicated \\
%     \hline
%     \end{tabular}
%     \label{tab:my_label}
% \end{table}

\begin{table}[]
    \centering
    \small
    \caption{\textcolor{red}{R2: Cross-domain}}
    \begin{tabular}{l|l|l}
    \hline
    \multirow{2}{*}{Dataset}  & \multicolumn{2}{c}{Domains} \\ \cline{2-3}
     & \multicolumn{1}{c|}{Visual} & \multicolumn{1}{c}{Textual} \\ \hline
    RefCOCO     & 80 classes & Positional + Short \\
    RefCOCO+    & 80 classes & Short \\
    RefCOCOg    & 80 classes & Long + Complicated \\
    PhraseCut   & 1203 classes & template \\
    \hline
    \end{tabular}
    \label{tab:my_label}
\end{table}


==> reb_tables/gt_mask_mscoco.tex <==
\begin{table}[h]
    \centering
    \footnotesize
    \caption{mIoU results of ETRIS model with full supervisions, GT segmentation masks with our generated pseudo text supervisions, and solely our pseudo-supervisions. S and T indicate GT segmentation masks and GT texts used for training. }
    \scalebox{0.9}{    
    \begin{tabular}{l|c|ccc|ccc}
    \hline
     \multirow{2}{*}{\makecell[l]{Supervision\\Types}} & \multirow{2}{*}{\makecell[c]{Human\\Label}}  & \multicolumn{3}{c|}{RefCOCO+} & \multicolumn{3}{c}{RefCOCOg} \\ \cline{3-8}
     & & val & testA  & testB & val(U) & test(U) & val(G) \\ \hline
     \multirow{1}{*}{\textit{Fully}} & S+T & 62.23 & 68.51 & 52.79 & 60.28 & 60.42 & 57.86 \\ \cdashline{1-8}[1pt/1pt]
     \multirow{4}{*}{\makecell[l]{\textit{Pseudo}\\(Ours)}} & S + T$^\dagger$ & 52.54 & 60.24 & 42.43 & 54.66 & 54.78 & 55.82 \\
     & S & 52.54 & 60.24 & 42.43 & 54.66 & 54.78 & 55.82 \\
     & T$^\dagger$ & 52.54 & 60.24 & 42.43 & 54.66 & 54.78 & 55.82 \\
      & - & 44.33 & 51.42 & 35.08 & 45.99 & 46.67 & 46.80 \\
    \hline
    
    \end{tabular}
    }
    \label{tab:mask_generator}
\end{table}

==> reb_tables/llava.tex <==
\vspace{-0.7cm}
\begin{table}[h]
    \centering
    \scriptsize
    \caption{\footnotesize{mIoU results of simply using LLAVA following InstructDET. We evaluate generated pseudo-supervisions using ETRIS in the rebuttal.}}
    \begin{tabular}{ll|ccc}
    \hline
    Models & Params  & RefCOCO & RefCOCO+ & RefCOCOg \\ \hline
    LLAVA  & 13B & 20.51 & 20.84 & 20.42 \\
    Ours (CoCa) & 2.1B & 41.05 & 44.33 & 45.99 \\ \hline
    % CLIPCAP & COCO & - & - & - \\ \hline
    \end{tabular}
    \label{reb_tab:llava}
\end{table}
\vspace{-0.2cm}

==> reb_tables/segmentation_masks.tex <==
\vspace{-0.6cm}
\begin{table}[h]
    \centering
    \scriptsize
    \caption{\footnotesize{Analysis on the impact of CutLER and SAM masks. $\dagger$ denotes that we heuristically reduce SAM masks to prevent OOM issues.}}
    \begin{tabular}{l|ccc}
    \hline
    Mask & RefCOCO & RefCOCO+ & RefCOCOg \\ \hline
    % \multirow{2}{*}{\textit{CutLER}}& & \textit{Zero-shot}~\cite{global_local_clip}  & 27.35 & 28.34 & 33.23 \\
    CutLER  & 37.40 & 39.42 & 42.63 \\
    SAM$^\dagger$ & 38.27 & 42.16 & 44.50 \\
    SAM + CutLER  & 41.05 & 44.33 & 45.99 \\
    % & & Ref-Diff & 37.21 & 37.29 & 44.02 \\
    % GT  & 47.22 & 52.54 & 54.66 \\ 
    \hline
    \end{tabular}
    \label{reb_tab:segmentation_masks}
\end{table}
\vspace{-0.3cm}

==> supple_tables/distinctiveness_datasets.tex <==
\begin{table}[h]
    \centering
    \footnotesize
    \caption{Caption}
    \begin{tabular}{c|ccc}
    \hline
         & RefCOCO & RefCOCO+ & RefCOCOg \\ \hline
    Distinctiveness     & 1.018 & 1.046 & 1.124 \\
    \hline
    \end{tabular}
    \label{sup_tab:distinctiveness_datasets}
\end{table}

==> tables/main_results.tex <==
\begin{table*}
    \tiny
    \centering
    \caption{Comparision with zero-shot and weakly-supervised RIS methods. Our pseudo supervised RIS models perform a zero-shot evaluation on RIS benchmark datasets. U and G denote UMD and Google splits of RefCOCOg, respectively. S and T are segmentation and text supervision by human.}
    \scalebox{0.9}{
    \begin{tabular}{c|l@{\hspace{8pt}}cll|ccc|ccc|ccc}
    \hline
    \multirow{2}{*}{Metric} &  \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Supervision\\ Types\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Human\\ Label\end{tabular}} & \multirow{2}{*}{Methods} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Mask\\ Gen.\end{tabular}}   & \multicolumn{3}{c|}{RefCOCO}  & \multicolumn{3}{c|}{RefCOCO+} & \multicolumn{3}{c}{RefCOCOg} \\ \cline{6-14}
       &  & &  &  & val   & testA    & testB    & val   & testA    & testB    & val(U)  & test(U) & val(G) \\ \hline
    \multirow{8}{*}{oIoU} & \multirow{2}{*}{\textit{Weakly}} & \multirow{2}{*}{T} &  SaG~\cite{shatter_and_gather} & & 30.40 & 29.75  &  31.24 &  25.27 & 24.46  & 26.04  & 27.12  &  - & - \\
    & &&TRIS~\cite{tris} &   & 28.12  & 28.68  & 27.68  & 28.33  & 27.20 & 29.00 &  33.63 & 33.89  & 33.24 \\
    \cline{2-14}
    &\multirow{2}{*}{\textit{Zero-shot}} & \multirow{2}{*}{-} &   Global-Local\cite{global_local_clip}  & SAM  & 24.55  & 26.00  & 21.03  & 26.62  & 29.99 & 22.23  & 28.92  &  30.48 & 30.19 \\
    && &   Ref-Diff~\cite{ref_diff}   & SAM & 35.16  &  37.44 & \textbf{34.50}  & 35.56  & 38.66  & 31.40  & 38.62 & 37.50 & 37.82 \\    \cdashline{2-14}[1pt/1pt]
    & \multirow{2}{*}{\textit{Pseudo}} &\multirow{2}{*}{-} &  Ours + CRIS   & SAM  & 35.45  & 39.69  & 30.37  & 37.55  & 41.52  & 31.71 & 37.90 & 39.64  & 39.32 \\
    & & &   Ours + ETRIS   & SAM  &  \textbf{37.33} & \textbf{43.43}  & 31.90  & \textbf{40.19}  & \textbf{46.43}  & \textbf{33.63} & \textbf{41.63} & \textbf{43.52}  & \textbf{42.97} \\ \cline{2-14}

    & \multirow{2}{*}{\textit{Fully}} &\multirow{2}{*}{S+T} &  CRIS~\cite{cris} &    & 67.35 & 71.54 & 62.16 & 57.94 & 64.05 & 48.42 & 56.56 & 57.38 & -  \\ 
    & & &  ETRIS~\cite{etris} &   & 69.36  & 72.68  & 63.68  & 58.59  & 66.93  & 50.14  & 58.62  & 60.12 & 55.56 \\
    \hline \hline
    

    \multirow{9}{*}{mIoU}& \multirow{3}{*}{\textit{Weakly}} &\multirow{3}{*}{T} &  Lee \textit{et al.}~\cite{weakly_ris_1} & & 31.06 & 32.30&30.11 &31.28 &32.11 & 30.13& 32.88 &- &- \\
    && & SaG~\cite{shatter_and_gather}  & & 34.76 &  34.58 & 35.01  & 28.48  & 28.60  & 27.98  & 28.87  & -  & - \\ 
    && & TRIS~\cite{tris} &   &  31.17 & 32.43  & 29.56  &  30.90 & 30.42 & 30.80 & 36.19  & 36.23  & 36.00 \\ 
    \cline{2-14}
    &\multirow{2}{*}{\textit{Zero-shot}} & \multirow{2}{*}{-} &   Global-Local~\cite{global_local_clip} & SAM  & 31.83  & 32.93  & 28.64  & 34.97 & 37.11 & 30.61  & 40.66  & 40.94  & 41.68 \\
    & &&   Ref-Diff~\cite{ref_diff}   & SAM & 37.21  & 38.40  & \textbf{37.19}  & 37.29  & 40.51  & 33.01  & 44.02 & 44.51 & 44.26 \\    \cdashline{2-14}[1pt/1pt]
    & \multirow{2}{*}{\textit{Pseudo}} &\multirow{2}{*}{-}&   Ours + CRIS   & SAM  & 39.75  & 44.77  &  32.99 & 42.15  & 46.28  & 34.54 & 43.73 & 43.37  & 43.78 \\
    & & &  Ours + ETRIS   & SAM  & \textbf{41.05}  & \textbf{48.19} & 33.48 & \textbf{44.33}  & \textbf{51.42}  & \textbf{35.08} & \textbf{45.99} & \textbf{46.67}  & \textbf{46.80} \\ \cline{2-14}
    &\multirow{2}{*}{\textit{Fully}} &\multirow{2}{*}{S+T} &  CRIS~\cite{cris} &  & 70.34 & 73.41 & 65.72 & 62.13 & 67.68 & 53.42 & 60.30 & 60.29 & - \\ 
    & & &  ETRIS~\cite{etris} &   & 71.06  & 74.11  & 66.66  & 62.23  & 68.51  & 52.79  & 60.28  & 60.42 & 57.86 \\

    \hline

    
    \end{tabular}
    \label{tab:main_results}
    }
\end{table*}

% \begin{table*}
%     \footnotesize
%     \centering
%     \caption{Comparision with zero-shot and weakly-supervised RIS methods. Our pseudo supervised RIS models perform a zero-shot evaluation on RIS benchmark datasets. U and G denote UMD and Google splits of RefCOCOg, respectively.}
%     \begin{tabular}{c|lll|ccc|ccc|ccc}
%     \hline
%     \multirow{2}{*}{Metric} &  \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Supervision\\ Types\end{tabular}} & \multirow{2}{*}{Methods} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Mask\\ Gen.\end{tabular}}   & \multicolumn{3}{c|}{RefCOCO}  & \multicolumn{3}{c|}{RefCOCO+} & \multicolumn{3}{c}{RefCOCOg} \\ \cline{5-13}
%        &  &   &  & val   & testA    & testB    & val   & testA    & testB    & val(U)  & test(U) & val(G) \\ \hline
%     % \multirow{14}{*}{oIoU}  &   ETRIS &  Full  &   &   &   &   &   &   &   & \\
%     % \multirow{11}{*}{oIoU}        &   \textbf{Weakly-supervised Method} &   &  & &   &   &   &   &   &   &    \\
%     \multirow{8}{*}{oIoU} & \multirow{2}{*}{\textit{Weakly} (T)} &   SaG~\cite{shatter_and_gather} & & 30.40 & 29.75  &  31.24 &  25.27 & 24.46  & 26.04  & 27.12  &  - & - \\
%     & &TRIS~\cite{tris} &   & 28.12  & 28.68  & 27.68  & 28.33  & 27.20 & 29.00 &  33.63 & 33.89  & 33.24 \\
%     \cline{2-13}
%     % &   \textbf{Zero-Shot Method}  &   &   &   &  & &   &   &   &   &    \\ 
%     % & \multirow{3}{*}{\textit{Zero-shot}} &   Global-Local~\cite{global_local_clip}   & FreeSOLO  & 24.88  & 23.61  & 24.66 & 26.16 & 24.90  & 25.83  & 31.11  & 30.96  & 30.69   \\ 
%     % &   Global-Local CLIP   & CutLER  & 24.01  & 25.29  & 23.61  & 24.90 & 25.84 & 25.08  & 28.06  & 29.32  & 29.08 \\
%     &\multirow{2}{*}{\textit{Zero-shot} (-)}  &   Global-Local\cite{global_local_clip}  & SAM  & 24.55  & 26.00  & 21.03  & 26.62  & 29.99 & 22.23  & 28.92  &  30.48 & 30.19 \\
%     % & & TAS & SAM & 29.53 & 30.26 & 28.24 & 33.21 & 38.77 & 28.01 & 35.84 & 36.16 & 36.36 \\
%     & &   Ref-Diff~\cite{ref_diff}   & SAM & 35.16  &  37.44 & \textbf{34.50}  & 35.56  & 38.66  & 31.40  & 38.62 & 37.50 & 37.82 \\    \cdashline{2-13}[1pt/1pt]
%     % &   Ours + CRIS    & CutLER  & 32.04  & 34.47  & 29.45  & 33.32  & 35.49 & 30.22 & 36.87  & 36.91  & 37.06 \\
%     % &   Ours + ETRIS    &  CutLER  & 33.87  & 37.04  & 30.42  & 36.80  & 40.05 & 32.55 & 38.94  & 38.67  & 39.08 \\    \cdashline{2-12}[1pt/1pt]
%     & \multirow{2}{*}{\textit{Pseudo} (-)} &   Ours + CRIS   & SAM  & 35.45  & 39.69  & 30.37  & 37.55  & 41.52  & 31.71 & 37.90 & 39.64  & 39.32 \\
%     & &   Ours + ETRIS   & SAM  &  \textbf{37.33} & \textbf{43.43}  & 31.90  & \textbf{40.19}  & \textbf{46.43}  & \textbf{33.63} & \textbf{41.63} & \textbf{43.52}  & \textbf{42.97} \\ \cline{2-13}
%      % & \textbf{Fully-supervised Method} &    &   &   &   &    &   &   &   &   &    \\
%     & \multirow{2}{*}{\textit{Fully} (S+T)} &   CRIS~\cite{cris} &    & 67.35 & 71.54 & 62.16 & 57.94 & 64.05 & 48.42 & 56.56 & 57.38 & -  \\ 
%     & &   ETRIS~\cite{etris} &   & 69.36  & 72.68  & 63.68  & 58.59  & 66.93  & 50.14  & 58.62  & 60.12 & 55.56 \\
%     \hline \hline
    
%     % \multirow{11}{*}{mIoU}     &   \textbf{Weakly-supervised Method} &   &  & &   &   &   &   &   &   &    \\
%     \multirow{9}{*}{mIoU}& \multirow{3}{*}{\textit{Weakly}} &  Lee \textit{et al.}~\cite{weakly_ris_1} & & 31.06 & 32.30&30.11 &31.28 &32.11 & 30.13& 32.88 &- &- \\
%     & & SaG~\cite{shatter_and_gather}  & & 34.76 &  34.58 & 35.01  & 28.48  & 28.60  & 27.98  & 28.87  & -  & - \\ 
%     & & TRIS~\cite{tris} &   &  31.17 & 32.43  & 29.56  &  30.90 & 30.42 & 30.80 & 36.19  & 36.23  & 36.00 \\ 
%     % & & SaG~\cite{shatter_and_gather}  & & 34.76 &  34.58 & 35.01  & 28.48  & 28.60  & 27.98  & 28.87  & -  & - \\ 
%     \cline{2-13}
%     % &   \textbf{Zero-Shot Method}  &   &   &   &  & &   &   &   &   &    \\ 
%     % & \multirow{3}{*}{\textit{Zero-shot}} &   Global-Local~\cite{global_local_clip}   & FreeSOLO  & 26.20  & 24.94  & 26.56 & 27.80 & 25.64  & 27.84  & 33.52  & 33.67  & 33.61   \\ 
%     % &   Global-Local CLIP   & CutLER  &  27.35 & 28.25  & 26.24  & 28.34 & 28.50 & 27.91  & 33.23  & 33.51  & 33.25 \\
%     &\multirow{2}{*}{\textit{Zero-shot}}  &   Global-Local~\cite{global_local_clip} & SAM  & 31.83  & 32.93  & 28.64  & 34.97 & 37.11 & 30.61  & 40.66  & 40.94  & 41.68 \\
%     % & & TAS & SAM & 39.84 & 41.08 & 36.24 & 43.63 & 49.13 & 36.54 & 46.62 & 46.80 & 48.05 \\
%     & &   Ref-Diff~\cite{ref_diff}   & SAM & 37.21  & 38.40  & \textbf{37.19}  & 37.29  & 40.51  & 33.01  & 44.02 & 44.51 & 44.26 \\    \cdashline{2-13}[1pt/1pt]
%     % &   Ours + CRIS     & CutLER  & 34.99  & 37.70 & 31.30  &  36.33 & 38.55 & 33.09 & 39.79  & 39.28  & 39.52 \\
%     % &   Ours + ETRIS    &  CutLER  & 37.40  & 41.20  & 32.49  & 39.42  & 42.76 & 34.21 & 42.63  & 41.67  & 42.24 \\    \cdashline{2-12}[1pt/1pt]
%     & \multirow{2}{*}{\textit{Pseudo}} &   Ours + CRIS   & SAM  & 39.75  & 44.77  &  32.99 & 42.15  & 46.28  & 34.54 & 43.73 & 43.37  & 43.78 \\
%     & &   Ours + ETRIS   & SAM  & \textbf{41.05}  & \textbf{48.19} & 33.48 & \textbf{44.33}  & \textbf{51.42}  & \textbf{35.08} & \textbf{45.99} & \textbf{46.67}  & \textbf{46.80} \\ \cline{2-13}
%         % & \textbf{Fully-supervised Method} &    &   &   &   &    &   &   &   &   &    \\
%     &\multirow{2}{*}{\textit{Fully}} &   CRIS~\cite{cris} &  & 70.34 & 73.41 & 65.72 & 62.13 & 67.68 & 53.42 & 60.30 & 60.29 & - \\ 
%     & &   ETRIS~\cite{etris} &   & 71.06  & 74.11  & 66.66  & 62.23  & 68.51  & 52.79  & 60.28  & 60.42 & 57.86 \\

%     \hline

    
%     \end{tabular}
%     \label{tab:main_results}
% \end{table*}

% \begin{table*}
%     \footnotesize
%     \centering
%     \caption{Comparision with zero-shot and weakly-supervised RIS methods. We perform a zero-shot evaluation on RIS benchmark datasets using our pseudo supervised RIS models. U and G denote UMD and Google splits of RefCOCOg, respectively.}
%     \begin{tabular}{c|ll|ccc|ccc|ccc}
%     \hline
%     \multirow{2}{*}{Metric} & \multirow{2}{*}{Methods}   & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Mask\\ Generator\end{tabular}}   & \multicolumn{3}{c|}{RefCOCO}  & \multicolumn{3}{c|}{RefCOCO+} & \multicolumn{3}{c}{RefCOCOg} \\ \cline{4-12}
%         &   &  & val   & test A    & test B    & val   & test A    & test B    & val(U)  & test(U) & val(G) \\ \hline
%     % \multirow{14}{*}{oIoU}  &   ETRIS &  Full  &   &   &   &   &   &   &   & \\
%     \multirow{11}{*}{oIoU} & \textbf{Fully-supervised Method} &    &   &   &   &    &   &   &   &   &    \\
%     &   CRIS~\cite{cris} &    & 67.35 & 71.54 & 62.16 & 57.94 & 64.05 & 48.42 & 56.56 & 57.38 & -  \\ 
%     &   ETRIS~\cite{etris} &   & 69.36  & 72.68  & 63.68  & 58.59  & 66.93  & 50.14  & 58.62  & 60.12 & 55.56 \\ \cline{2-12}
%     &   \textbf{Zero-Shot Method}  &   &   &   &  & &   &   &   &   &    \\ 
%     &   Global-Local CLIP~\cite{global_local_clip}   & FreeSOLO  & 24.88  & 23.61  & 24.66 & 26.16 & 24.90  & 25.83  & 31.11  & 30.96  & 30.69   \\ 
%     % &   Global-Local CLIP   & CutLER  & 24.01  & 25.29  & 23.61  & 24.90 & 25.84 & 25.08  & 28.06  & 29.32  & 29.08 \\
%     &   Global-Local CLIP\cite{global_local_clip}  & SAM  & 24.55  & 26.00  & 21.03  & 26.62  & 29.99 & 22.23  & 28.92  &  30.48 & 30.19 \\
%     & TAS & SAM & 29.53 & 30.26 & 28.24 & 33.21 & 38.77 & 28.01 & 35.84 & 36.16 & 36.36 \\
%     &   Ref-Diff~\cite{ref_diff}   & SAM & 35.16  &  37.44 & \textbf{34.50}  & 35.56  & 38.66  & 31.40  & 38.62 & 37.50 & 37.82 \\    \cdashline{2-12}[1pt/1pt]
%     % &   Ours + CRIS    & CutLER  & 32.04  & 34.47  & 29.45  & 33.32  & 35.49 & 30.22 & 36.87  & 36.91  & 37.06 \\
%     % &   Ours + ETRIS    &  CutLER  & 33.87  & 37.04  & 30.42  & 36.80  & 40.05 & 32.55 & 38.94  & 38.67  & 39.08 \\    \cdashline{2-12}[1pt/1pt]
%     &   Ours + CRIS   & SAM  & 35.45  & 39.69  & 30.37  & 37.55  & 41.52  & 31.71 & 37.90 & 39.64  & 39.32 \\
%     &   Ours + ETRIS   & SAM  &  \textbf{37.33} & \textbf{43.43}  & 31.90  & \textbf{40.19}  & \textbf{46.43}  & \textbf{33.63} & \textbf{41.63} & \textbf{43.52}  & \textbf{42.97} \\ \cline{2-12}
%         &   \textbf{Weakly-supervised Method} &   &  & &   &   &   &   &   &   &    \\
%     &   Shatter and Gather~\cite{shatter_and_gather} & & 30.40 & -  &  - &  - & -  & -  & -  &  - & - \\ 
%     &   TRIS~\cite{tris} &   & 28.12  & 28.68  & 27.68  & 28.33  & 27.20 & 29.00 &  33.63 & 33.89  & 33.24 \\
%     \hline \hline
    
%     \multirow{11}{*}{mIoU} & \textbf{Fully-supervised Method} &    &   &   &   &    &   &   &   &   &    \\
%     &   CRIS~\cite{cris} &  & 70.34 & 73.41 & 65.72 & 62.13 & 67.68 & 53.42 & 60.30 & 60.29 & - \\ 
%     &   ETRIS~\cite{etris} &   & 71.06  & 74.11  & 66.66  & 62.23  & 68.51  & 52.79  & 60.28  & 60.42 & 57.86 \\ \cline{2-12}
%     &   \textbf{Zero-Shot Method}  &   &   &   &  & &   &   &   &   &    \\ 
%     &   Global-Local CLIP~\cite{global_local_clip}   & FreeSOLO  & 26.20  & 24.94  & 26.56 & 27.80 & 25.64  & 27.84  & 33.52  & 33.67  & 33.61   \\ 
%     % &   Global-Local CLIP   & CutLER  &  27.35 & 28.25  & 26.24  & 28.34 & 28.50 & 27.91  & 33.23  & 33.51  & 33.25 \\
%     &   Global-Local CLIP~\cite{global_local_clip} & SAM  & 31.83  & 32.93  & 28.64  & 34.97 & 37.11 & 30.61  & 40.66  & 40.94  & 41.68 \\
%     & TAS & SAM & 39.84 & 41.08 & 36.24 & 43.63 & 49.13 & 36.54 & 46.62 & 46.80 & 48.05 \\
%     &   Ref-Diff~\cite{ref_diff}   & SAM & 37.21  & 38.40  & \textbf{37.19}  & 37.29  & 40.51  & 33.01  & 44.02 & 44.51 & 44.26 \\    \cdashline{2-12}[1pt/1pt]
%     % &   Ours + CRIS     & CutLER  & 34.99  & 37.70 & 31.30  &  36.33 & 38.55 & 33.09 & 39.79  & 39.28  & 39.52 \\
%     % &   Ours + ETRIS    &  CutLER  & 37.40  & 41.20  & 32.49  & 39.42  & 42.76 & 34.21 & 42.63  & 41.67  & 42.24 \\    \cdashline{2-12}[1pt/1pt]
%     &   Ours + CRIS   & SAM  & 39.75  & 44.77  &  32.99 & 42.15  & 46.28  & 34.54 & 43.73 & 43.37  & 43.78 \\
%     &   Ours + ETRIS   & SAM  & \textbf{41.05}  & \textbf{48.19} & 33.48 & \textbf{44.33}  & \textbf{51.42}  & \textbf{35.08} & \textbf{45.99} & \textbf{46.67}  & \textbf{46.80} \\ \cline{2-12}
%     &   \textbf{Weakly-supervised Method} &   &  & &   &   &   &   &   &   &    \\
%     &   Shatter and Gather~\cite{shatter_and_gather} & & 34.76 &  34.58 & 35.01  & 28.48  & 28.60  & 27.98  & 28.87  & -  & - \\ 
%     &   TRIS~\cite{tris} &   &  31.17 & 32.43  & 29.56  &  30.90 & 30.42 & 30.80 & 36.19  & 36.23  & 36.00 \\
%     \hline

    
%     \end{tabular}
%     \label{tab:main_results}
% \end{table*}

% \begin{table*}
%     \scriptsize
%     \centering
%     \caption{Comparision with zero-shot and weakly-supervised RIS methods. We perform a zero-shot evaluation on RIS benchmark datasets using our pseudo supervised RIS models. U and G denote UMD and Google splits of RefCOCOg, respectively.}
%     \begin{tabular}{c|ll|ccc|ccc|ccc}
%     \hline
%     \multirow{2}{*}{Metric} & \multirow{2}{*}{Methods} & \multirow{2}{*}{Methods}   & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Mask\\ Generator\end{tabular}}   & \multicolumn{3}{c|}{RefCOCO}  & \multicolumn{3}{c|}{RefCOCO+} & \multicolumn{3}{c}{RefCOCOg} \\ \cline{4-12}
%         &   &  & val   & test A    & test B    & val   & test A    & test B    & val(U)  & test(U) & val(G) \\ \hline
%     % \multirow{14}{*}{oIoU}  &   ETRIS &  Full  &   &   &   &   &   &   &   & \\
%     \multirow{11}{*}{oIoU}        &   \textbf{Weakly-supervised Method} &   &  & &   &   &   &   &   &   &    \\
%     &   Shatter and Gather~\cite{shatter_and_gather} & & 30.40 & -  &  - &  - & -  & -  & -  &  - & - \\ 
%     &   TRIS~\cite{tris} &   & 28.12  & 28.68  & 27.68  & 28.33  & 27.20 & 29.00 &  33.63 & 33.89  & 33.24 \\ \cline{2-12}
%     &   \textbf{Zero-Shot Method}  &   &   &   &  & &   &   &   &   &    \\ 
%     &   Global-Local CLIP~\cite{global_local_clip}   & FreeSOLO  & 24.88  & 23.61  & 24.66 & 26.16 & 24.90  & 25.83  & 31.11  & 30.96  & 30.69   \\ 
%     % &   Global-Local CLIP   & CutLER  & 24.01  & 25.29  & 23.61  & 24.90 & 25.84 & 25.08  & 28.06  & 29.32  & 29.08 \\
%     &   Global-Local CLIP\cite{global_local_clip}  & SAM  & 24.55  & 26.00  & 21.03  & 26.62  & 29.99 & 22.23  & 28.92  &  30.48 & 30.19 \\
%     % & TAS & SAM & 29.53 & 30.26 & 28.24 & 33.21 & 38.77 & 28.01 & 35.84 & 36.16 & 36.36 \\
%     &   Ref-Diff~\cite{ref_diff}   & SAM & 35.16  &  37.44 & \textbf{34.50}  & 35.56  & 38.66  & 31.40  & 38.62 & 37.50 & 37.82 \\    \cdashline{2-12}[1pt/1pt]
%     % &   Ours + CRIS    & CutLER  & 32.04  & 34.47  & 29.45  & 33.32  & 35.49 & 30.22 & 36.87  & 36.91  & 37.06 \\
%     % &   Ours + ETRIS    &  CutLER  & 33.87  & 37.04  & 30.42  & 36.80  & 40.05 & 32.55 & 38.94  & 38.67  & 39.08 \\    \cdashline{2-12}[1pt/1pt]
%     &   Ours + CRIS   & SAM  & 35.45  & 39.69  & 30.37  & 37.55  & 41.52  & 31.71 & 37.90 & 39.64  & 39.32 \\
%     &   Ours + ETRIS   & SAM  &  \textbf{37.33} & \textbf{43.43}  & 31.90  & \textbf{40.19}  & \textbf{46.43}  & \textbf{33.63} & \textbf{41.63} & \textbf{43.52}  & \textbf{42.97} \\ \cline{2-12}
%      & \textbf{Fully-supervised Method} &    &   &   &   &    &   &   &   &   &    \\
%     &   CRIS~\cite{cris} &    & 67.35 & 71.54 & 62.16 & 57.94 & 64.05 & 48.42 & 56.56 & 57.38 & -  \\ 
%     &   ETRIS~\cite{etris} &   & 69.36  & 72.68  & 63.68  & 58.59  & 66.93  & 50.14  & 58.62  & 60.12 & 55.56 \\
%     \hline \hline
    
%     \multirow{11}{*}{mIoU}     &   \textbf{Weakly-supervised Method} &   &  & &   &   &   &   &   &   &    \\
%     &   Shatter and Gather~\cite{shatter_and_gather} & & 34.76 &  34.58 & 35.01  & 28.48  & 28.60  & 27.98  & 28.87  & -  & - \\ 
%     &   TRIS~\cite{tris} &   &  31.17 & 32.43  & 29.56  &  30.90 & 30.42 & 30.80 & 36.19  & 36.23  & 36.00 \\ \cline{2-12}
%     &   \textbf{Zero-Shot Method}  &   &   &   &  & &   &   &   &   &    \\ 
%     &   Global-Local CLIP~\cite{global_local_clip}   & FreeSOLO  & 26.20  & 24.94  & 26.56 & 27.80 & 25.64  & 27.84  & 33.52  & 33.67  & 33.61   \\ 
%     % &   Global-Local CLIP   & CutLER  &  27.35 & 28.25  & 26.24  & 28.34 & 28.50 & 27.91  & 33.23  & 33.51  & 33.25 \\
%     &   Global-Local CLIP~\cite{global_local_clip} & SAM  & 31.83  & 32.93  & 28.64  & 34.97 & 37.11 & 30.61  & 40.66  & 40.94  & 41.68 \\
%     % & TAS & SAM & 39.84 & 41.08 & 36.24 & 43.63 & 49.13 & 36.54 & 46.62 & 46.80 & 48.05 \\
%     &   Ref-Diff~\cite{ref_diff}   & SAM & 37.21  & 38.40  & \textbf{37.19}  & 37.29  & 40.51  & 33.01  & 44.02 & 44.51 & 44.26 \\    \cdashline{2-12}[1pt/1pt]
%     % &   Ours + CRIS     & CutLER  & 34.99  & 37.70 & 31.30  &  36.33 & 38.55 & 33.09 & 39.79  & 39.28  & 39.52 \\
%     % &   Ours + ETRIS    &  CutLER  & 37.40  & 41.20  & 32.49  & 39.42  & 42.76 & 34.21 & 42.63  & 41.67  & 42.24 \\    \cdashline{2-12}[1pt/1pt]
%     &   Ours + CRIS   & SAM  & 39.75  & 44.77  &  32.99 & 42.15  & 46.28  & 34.54 & 43.73 & 43.37  & 43.78 \\
%     &   Ours + ETRIS   & SAM  & \textbf{41.05}  & \textbf{48.19} & 33.48 & \textbf{44.33}  & \textbf{51.42}  & \textbf{35.08} & \textbf{45.99} & \textbf{46.67}  & \textbf{46.80} \\ \cline{2-12}
%         & \textbf{Fully-supervised Method} &    &   &   &   &    &   &   &   &   &    \\
%     &   CRIS~\cite{cris} &  & 70.34 & 73.41 & 65.72 & 62.13 & 67.68 & 53.42 & 60.30 & 60.29 & - \\ 
%     &   ETRIS~\cite{etris} &   & 71.06  & 74.11  & 66.66  & 62.23  & 68.51  & 52.79  & 60.28  & 60.42 & 57.86 \\

%     \hline

    
%     \end{tabular}
%     \label{tab:main_results}
% \end{table*}



% \begin{table*}
%     \footnotesize
%     \centering
%     \caption{Caption}
%     \begin{tabular}{c|ll|ccc|ccc|ccc}
%     \hline
%     \multirow{2}{*}{Metric} & \multirow{2}{*}{Methods}   & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Mask\\ Generator\end{tabular}}   & \multicolumn{3}{c|}{RefCOCO}  & \multicolumn{3}{c|}{RefCOCO+} & \multicolumn{3}{c}{RefCOCOg} \\ \cline{4-12}
%         &   &  & val   & test A    & test B    & val   & test A    & test B    & val(U)  & test(U) & test(G) \\ \hline
%     % \multirow{14}{*}{oIoU}  &   ETRIS &  Full  &   &   &   &   &   &   &   & \\
%     \multirow{14}{*}{oIoU} & \textbf{Fully-supervised Method} &    &   &   &   &    &   &   &   &   &    \\
%     &   CRIS &    & 67.35 & 71.54 & 62.16 & 57.94 & 64.05 & 48.42 & 56.56 & 57.38 & -  \\ 
%     &   ETRIS &   & 69.36  & 72.68  & 63.68  & 58.59  & 66.93  & 50.14  & 58.62  & 60.12 & 55.56 \\ \cline{2-12}
%     &   \textbf{Zero-Shot Method}  &   &   &   &  & &   &   &   &   &    \\ 
%     &   Global-Local CLIP   & FreeSOLO  & 24.88  & 23.61  & 24.66 & 26.16 & 24.90  & 25.83  & 31.11  & 30.96  & 30.69   \\ 
%     &   Global-Local CLIP   & CutLER  & 24.01  & 25.29  & 23.61  & 24.90 & 25.84 & 25.08  & 28.06  & 29.32  & 29.08 \\
%     &   Global-Local CLIP   & SAM  & 24.55  & 26.00  & 21.03  & 26.62  & 29.99 & 22.23  & 28.92  &  30.48 & 30.19 \\
%     &   Ref-Diff   & SAM & 35.16  &  37.44 & 34.50  & 35.56  & 38.66  & 31.40  & 38.62 & 37.50 & 37.82 \\    \cdashline{2-12}[1pt/1pt]
%     &   Ours + CRIS    & CutLER  & 32.04  & 34.47  & 29.45  & 33.32  & 35.49 & 30.22 & 36.87  & 36.91  & 37.06 \\
%     &   Ours + ETRIS    &  CutLER  & 33.87  & 37.04  & 30.42  & 36.80  & 40.05 & 32.55 & 38.94  & 38.67  & 39.08 \\    \cdashline{2-12}[1pt/1pt]
%     &   Ours + CRIS   & SAM  & 35.45  & 39.69  & 30.37  & 37.55  & 41.52  & 31.71 & 37.90 & 39.64  & 39.32 \\
%     &   Ours + ETRIS   & SAM  &  \textbf{37.33} & 43.43  & 31.90  & \textbf{40.19}  & 46.43  & 33.63 & \textbf{41.63} & 43.52  & 42.97 \\ \cline{2-12}
%         &   \textbf{Weakly-supervised Method} &   &  & &   &   &   &   &   &   &    \\
%     &   Shatter and Gather & & 30.40 & -  &  - &  - & -  & -  & -  &  - & - \\ 
%     &   TRIS &   & -  & -  & -  & -  & - & - &  - & -  & - \\
%     \hline \hline
    
%     \multirow{14}{*}{mIoU} & \textbf{Fully-supervised Method} &    &   &   &   &    &   &   &   &   &    \\
%     &   CRIS &  & 70.34 & 73.41 & 65.72 & 62.13 & 67.68 & 53.42 & 60.30 & 60.29 & - \\ 
%     &   ETRIS &   & 71.06  & 74.11  & 66.66  & 62.23  & 68.51  & 52.79  & 60.28  & 60.42 & 57.86 \\ \cline{2-12}
%     &   \textbf{Zero-Shot Method}  &   &   &   &  & &   &   &   &   &    \\ 
%     &   Global-Local CLIP   & FreeSOLO  & 26.20  & 24.94  & 26.56 & 27.80 & 25.64  & 27.84  & 33.52  & 33.67  & 33.61   \\ 
%     &   Global-Local CLIP   & CutLER  &  27.35 & 28.25  & 26.24  & 28.34 & 28.50 & 27.91  & 33.23  & 33.51  & 33.25 \\
%     &   Global-Local CLIP   & SAM  & 31.83  & 32.93  & 28.64  & 34.97 & 37.11 & 30.61  & 40.66  & 40.94  & 41.68 \\
%     &   Ref-Diff   & SAM & 37.21  & 38.40  & \textbf{37.19}  & 37.29  & 40.51  & 33.01  & 44.02 & 44.51 & 44.26 \\    \cdashline{2-12}[1pt/1pt]
%     &   Ours + CRIS     & CutLER  & 34.99  & 37.70 & 31.30  &  36.33 & 38.55 & 33.09 & 39.79  & 39.28  & 39.52 \\
%     &   Ours + ETRIS    &  CutLER  & 37.40  & 41.20  & 32.49  & 39.42  & 42.76 & 34.21 & 42.63  & 41.67  & 42.24 \\    \cdashline{2-12}[1pt/1pt]
%     &   Ours + CRIS   & SAM  & 39.75  & 44.77  &  32.99 & 42.15  & 46.28  & 34.54 & 43.73 & 43.37  & 43.78 \\
%     &   Ours + ETRIS   & SAM  & \textbf{41.05}  & \textbf{48.19} & 33.48 & \textbf{44.33}  & \textbf{51.42}  & \textbf{35.08} & \textbf{45.99} & \textbf{46.67}  & \textbf{ 46.80} \\ \cline{2-12}
%     &   \textbf{Weakly-supervised Method} &   &  & &   &   &   &   &   &   &    \\
%     &   Shatter and Gather & & 34.76 &  34.58 & 35.01  & 28.48  & 28.60  & 27.98  & 28.87  & -  & - \\ 
%     &   TRIS &   &  31.17 & 32.43  & 29.56  &  30.90 & 30.42 & 30.80 & 36.19  & 36.23  & 36.00 \\
%     \hline

    
%     \end{tabular}
%     \label{tab:main_results}
% \end{table*}
    
% \begin{table*}[ht!]
% \footnotesize
% \centering
%     \caption{Comparison with Zero-shot RIS baseline methods on three standard benchmark datasets. U: The UMD partition. G: The Google partition. All baseline methods use FreeSOLO as the mask proposal network. $\dag$ denotes that the model is initialized with the ImageNet pre-trained weights and trained on RIS datasets. FreeSOLO upper-bound is computed between the GT mask and the maximum overlapped FreeSOLO mask with the GT mask.}
%     % max overall IoU Mask of FreeSOLO outputs and GT mask 


% \begin{tabular}{c|ll|ccc|ccc|ccc}
% \hline
% \multirow{2}{*}{Metric} & \multirow{2}{*}{Methods}            & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Visual\\ Encoder\end{tabular}} & \multicolumn{3}{c|}{RefCOCO}                     & \multicolumn{3}{c|}{RefCOCO+}                    & \multicolumn{3}{c}{RefCOCOg}                     \\ \cline{4-12} 
% & &     & val            & test A         & test B         & val            & test A         & test B         & val(U)            & test(U)        & val(G)         \\ \hline
% \multirow{10}{*}{oIoU} & Supervised SoTA method~\cite{lavt} &                                                                           &    72.73            &    75.82            &   68.79             &  62.14              &   68.38             &    55.10            &     61.24           &    62.09            &   60.50             \\ \cline{2-12}
% & \textbf{Zero-Shot Baselines} &                                                                           &                &                &                &                &                &                &                &                &                \\
% & Grad-CAM                     & ResNet-50                                                                 & 14.02          & 15.07          & 13.49          & 14.46          & 14.97          & 14.04          & 12.51          & 12.81          & 12.86          \\
% & Score map                     & ResNet-50                                                                 & 19.87          & 19.31          & 20.22          & 20.37          & 19.65          & 20.75          & 18.88          & 19.16          & 19.15          \\
% & Region token                & ViT-B/32                                                                  & 21.71          & 20.31          & 22.63          & 22.61          & 20.91          & 23.46          & 25.52          & 25.38          & 25.29          \\
% & Cropping                    & ResNet-50                                                                 & 22.36          & 20.49          & 22.69          & 23.95          & 22.03          & 23.49          & 28.20          & 27.64          & 27.47          \\
% & Cropping                      & ViT-B/32                                                                  & 22.73          & 21.11          & 23.08          & 24.09          & 22.42          & 23.93          & 28.69          & 27.51          & 27.70          \\ \cline{2-12}
% & Global-Local CLIP (ours)                         & ResNet-50                                                                 & 24.58          & 23.38          & 24.35          & 25.87          & 24.61          & 25.61          & 30.07          & 29.83          & 29.45          \\
% & Global-Local CLIP (ours)                         & ViT-B/32                                                                  & \textbf{24.88} & \textbf{23.61} & \textbf{24.66} & \textbf{26.16} & \textbf{24.90} & \textbf{25.83} & \textbf{31.11} & \textbf{30.96} & \textbf{30.69} \\ 
% \cdashline{2-12}[1pt/1pt]
% & FreeSOLO upper-bound         & \multicolumn{1}{c|}{-}                                                    & 42.08          & 42.52          & 43.52          & 42.17          & 42.52          & 43.80          & 48.81          & 48.96          & 48.49          \\ 
% \hline
% \hline
% \multirow{11}{*}{mIoU} & \textbf{Zero-Shot Baselines} &                                                                           &                &                &                &                &                &                &                &                &                \\
% & Grad-CAM                    & ResNet-50                                                                 & 14.22          & 15.93          & 13.18          & 14.80         & 15.87          & 13.78        & 12.47          & 13.16          & 13.30          \\
% & Score map                    & ResNet-50                                                                 & 21.32          & 20.96          & 21.57          & 21.61          & 21.17          & 22.30          & 20.07          & 20.43          & 20.63          \\
% & Region token               & ViT-B/32                                                                  & 23.43          & 22.07          & 24.62          & 24.51          & 22.64          & 25.37          & 27.57          & 27.34          & 27.69          \\
% & Cropping                 & ResNet-50                                                                 & 24.31          & 22.37          & 24.66          & 26.31          & 23.94          & 25.69          & 31.27          & 30.87          & 30.78          \\
% & Cropping                 & ViT-B/32                                                                  & 24.83          & 22.58          & 25.72          & 26.33          & 24.06          & 26.46          & 31.88          & 30.94          & 31.06          \\ \cline{2-12}
% & Global-Local CLIP (ours)            & ResNet-50                                                                 & \textbf{26.70} & \textbf{24.99} & 26.48          & \textbf{28.22} & \textbf{26.54} & \textbf{27.86} & 33.02          & 33.12          & 32.79          \\
% & Global-Local CLIP (ours)            & ViT-B/32                                                                  & 26.20          & 24.94          & \textbf{26.56} & 27.80          & 25.64          & 27.84          & \textbf{33.52} & \textbf{33.67} & \textbf{33.61} \\ 
% \cdashline{2-12}[1pt/1pt]
% & FreeSOLO upper-bound                & \multicolumn{1}{c|}{-}                                                    & 48.25          & 46.62          & 50.43          & 48.28          & 46.62          & 50.62          & 52.44          & 52.91          & 52.76          \\ \cline{2-12}
% & \textbf{Weakly-supervised method}   &                                                                           &                &                &                &                &                &                &                &                &                \\
% & TSEG~\cite{tseg}                        & ViT-S/16$^\dagger$                                                        & 25.95          & -              & -              & 22.62          & -              & -              & 23.41          & -              & -              \\ \hline
% \end{tabular}
% \label{tab:total}

% \end{table*}

==> tables/semi_miou_results.tex <==
\begin{table*}
    \footnotesize
    \centering
    \caption{Caption}
    \begin{tabular}{l|ccc|ccc|ccc}
    \hline
    \multirow{2}{*}{Method} & \multicolumn{3}{c|}{RefCOCO}  & \multicolumn{3}{c|}{RefCOCO+} & \multicolumn{3}{c}{RefCOCOg} \\ \cline{3-11}
       & val   & test A    & test B    & val   & test A    & test B    & val(U)  & test(U) & test(G) \\ \hline
    % \multirow{14}{*}{oIoU}  &   ETRIS &  Full  &   &   &   &   &   &   &   & \\
    \multicolumn{1}{c|}{\textbf{0.1\% Training}}   &   &   &   &    &   &   &   &   &    \\
    Supervised    & &  &  &  &  &  &  &  &   \\ 
    % &   CRIS + Ours  & 69.36  & 72.68  & 63.68  & 58.59  & 66.93  & 50.14  & 58.62  & 60.12 & 55.56 \\
    Ours & &  &  &  &  &  &  &  &   \\  \cdashline{2-11}[1pt/1pt]
    \multicolumn{1}{c|}{\textbf{1\% Training}}  &   &   &   &  &   &   &   &   &    \\ 
    Supervised   & &  &  &  &  &  &  &  &   \\ 
    % &   CRIS + Ours  & 69.36  & 72.68  & 63.68  & 58.59  & 66.93  & 50.14  & 58.62  & 60.12 & 55.56 \\
    Ours & &  &  &  &  &  &  &  &   \\  \cdashline{2-11}[1pt/1pt]
    \multicolumn{1}{c|}{\textbf{5\% Training}}    &   &   &  & &   &   &   &   &    \\ 
    Supervised    & &  &  &  &  &  &  &  &   \\ 
    % &   CRIS + Ours  & 69.36  & 72.68  & 63.68  & 58.59  & 66.93  & 50.14  & 58.62  & 60.12 & 55.56 \\
    Ours & &  &  &  &  &  &  &  &   \\  \cdashline{2-11}[1pt/1pt]
    \multicolumn{1}{c|}{\textbf{10\% Training}}  &   &   &  & &   &   &   &   &    \\ 
    Supervised    & &  &  &  &  &  &  &  &   \\ 
    % &   CRIS + Ours  & 69.36  & 72.68  & 63.68  & 58.59  & 66.93  & 50.14  & 58.62  & 60.12 & 55.56 \\
    Ours & &  &  &  &  &  &  &  &   \\ 
    \hline 

    \end{tabular}
    \label{tab:semi_miou_results}
\end{table*}

==> tables/semi_refcocog.tex <==
\begin{table}[]
    \centering
    \small
    \begin{tabular}{l|l|ccc}
    \hline
         Method & Additional & val(U) & test(U) & val(G)\\ \hline
         CRIS & - & & & \\
         CRIS & Ours & & & \\ \cdashline{1-5}[1pt/1pt]
         ETRIS & - & 60.28 & 60.42 & 57.86 \\
         ETRIS & Ours & 61.66 & 62.02 & 58.73 \\ \hline
    \end{tabular}
    \caption{mIoU results on RefCOCOg with additional data. We use our pseudo supervision as additional training.}
    \label{tab:semi_refcocog}
\end{table}

==> tables/urs.tex <==
% \begin{table}[]
%     \centering
%     \small
%     \caption{Average Uniquely Referring Score (URS) results when using Distinctive Sampling with different mask generators. URS is dependent on mask quality. Improving URS scores by using DS shows }
%     \begin{tabular}{l|c@{\hspace{0.5em}}c@{\hspace{0.5em}}c}
%         \hline
%         Pseudo & \multicolumn{3}{c}{Sampling Method} \\ \cline{2-4}
%         Supervision & Standard & & Distinctive\\ \hline
%         {\footnotesize with} CutLER & 1.189 & $\rightarrow$ & 1.308 \\
%         {\footnotesize with} SAM & 1.081 & $\rightarrow$ & 1.156 \\ \hline
%     \end{tabular}
%     \label{tab:urs_on_ds}
% \end{table}

\begin{table}[]
    \centering
    \small
    \caption{Average Uniquely Referring Score (URS) results when using Distinctive Sampling with different mask generators. URS is dependent on mask quality. Improving URS scores by using DS shows }
    \begin{tabular}{l|c@{\hspace{0.5em}}c@{\hspace{0.5em}}c}
        \hline
        % & \multicolumn{3}{c}{Sampling Method} \\ \cline{2-4}
        & Standard Sampling & & Distinctive Sampling \\ \hline
        % &Sampling & & Sampling \\ \hline
        % {\footnotesize with} CutLER & 1.189 & $\rightarrow$ & 1.308 \\
        URS & 1.081 & $\rightarrow$ & 1.156 \\ \hline
    \end{tabular}
    \label{tab:urs_on_ds}
\end{table}
